Heterogeneous Federated Learning using Dynamic Model Pruning and Adaptive Gradient

Federated Learning (FL) has emerged as a new paradigm for training machine learning models distributively without sacrificing data security and privacy. Learning models on edge devices such as mobile phones is one of the most common use cases for FL. However, Non-identical independent distributed~(non-IID) data in edge devices easily leads to training failures. Especially, over-parameterized machine learning models can easily be over-fitted on such data, hence, resulting in inefficient federated learning and poor model performance. To overcome the over-fitting issue, we proposed an adaptive dynamic pruning approach for FL, which can dynamically slim the model by dropping out unimportant parameters, hence, preventing over-fittings. Since the machine learning model's parameters react differently for different training samples, adaptive dynamic pruning will evaluate the salience of the model's parameter according to the input training sample, and only retain the salient parameter's gradients when doing back-propagation. We performed comprehensive experiments to evaluate our approach. The results show that our approach by removing the redundant parameters in neural networks can significantly reduce the over-fitting issue and greatly improves the training efficiency. In particular, when training the ResNet-32 on CIFAR-10, our approach reduces the communication cost by 57\%. We further demonstrate the inference acceleration capability of the proposed algorithm. Our approach reduces up to 50\% FLOPs inference of DNNs on edge devices while maintaining the model's quality.

==> Content/a01_federated_dynamic.tex <==

\begin{algorithm}[H]

    \caption{Dataset-aware dynamic pruning with \emph{FedAvg}, \textcolor{blue}{\emph{FedProx}}, \textcolor{red}{\emph{FedNova}}}
    \label{alg_fed_dp}
\begin{algorithmic}

\STATE {\bfseries Input:} $K$ clients indexed by $k$, number of communication rounds $T$, number of local epochs $E$, learning rate $\eta$, total number of samples $n$, number of sample in $k^{th}$ client $n_k$.
\STATE {\bfseries Output:} final model $w^T$.

\STATE


\STATE {\bfseries Server executes:} 
\STATE initialize $w^0$
\FOR{each round $t =1,2,\dots, T$}
    
    \STATE $K \leftarrow$ random set of clients
    \FOR{each client $k \in K$ {\bfseries in parallel}}
        \STATE send $w^{t}$ to client $k$
        \IF{method = \emph{FedAvg} || \textcolor{blue}{\emph{FedProx}} }{
            \STATE $\hat{w}^{t+1}_k\leftarrow$ ClientUpdate$(k,w^t)$
        }
        \ENDIF
        \IF {method = \textcolor{red}{\emph{FedNova}} }{
            \STATE $\hat{w}^{t+1}_k,\textcolor{red}{\tau_{k}}\leftarrow$ ClientUpdate$(k,w^t)$
        }
        \ENDIF
    \ENDFOR
    
    % \STATE $w_{t+1} \leftarrow \sum\limits_{c\in C} \alpha_c w_{t+1}^c $
    % \STATE initialize $w^{t+1}$ with zero matrix
    % \FOR{each client $k \in K$}
        \IF{method = \emph{FedAvg} || \textcolor{blue}{\emph{FedProx}} }{
            
            \STATE $w^{t+1} \leftarrow  w^{t} + \sum_{k=1}^{K}\frac{n_k}{n} \hat{w}^{t}_k $   
            % \# with \emph{FedAvg} and \textcolor{blue}{\emph{FedProx}}
            }
        \ENDIF
        \IF {method = \textcolor{red}{\emph{FedNova}} }{
            \STATE $w^{t+1} \leftarrow  w^{t} \textcolor{red}{-\eta \frac{\sum_{k=1}^{K} n_k {\tau_{k}}}{n}} \sum_{k=1}^{K}\frac{n_k}{n\textcolor{red}{\tau_{k}}} \hat{w}^{t}_k $ 
            % \# with \textcolor{red}{\emph{FedNova}} 
        }
        \ENDIF
        
        % \SWITCH{method}
        %     \CASE{\emph{FedAvg}}
        %         $w_{t+1} \leftarrow  w_{t+1} + \sum_{c=1}^{m}\frac{n_c}{n} \hat{w}_{t+1}^c $   
        %     \ENDCASE
        %     \CASE{\textcolor{blue}{\emph{FedProx}}}
        %         $w_{t+1} \leftarrow  w_{t+1} + \textcolor{red}{\frac{\sum_{c=1}^{m} n_c {\tau^{c}}}{n}} \sum_{c=1}^{m}\frac{n_c}{n\textcolor{red}{\tau^{c}}} \hat{w}_{t+1}^c $ 
        %     \ENDCASE
        % \ENDSWITCH
        
        
    % \ENDFOR
\ENDFOR

% \STATE {\bfseries Client executes (Loss function):} 

%     \# \textcolor{blue}{\emph{FedAvg}} and \textcolor{cyan}{\emph{FedNova}}

%     \# \textcolor{cyan}{\emph{FedProx}},

\STATE
\STATE {\bfseries ClientUpdate($k, w^t$):}
\STATE $\mathcal{B} \leftarrow$ split local dataset into batches 
\STATE $w_k^t \leftarrow$ download global model parameter $w^t$

\IF{method = \emph{FedAvg} || \textcolor{red}{\emph{FedNova}} }{
    \STATE $\mathcal{L}(w,w_g;b) = \sum_{(x,y) \in b}l(w;x;y)$
    }
\ENDIF
\IF {method = \textcolor{blue}{\emph{FedProx}} } {
    \STATE $\mathcal{L}(w,w_g;b) = \sum_{(x,y) \in b}l(w;x;y) + \textcolor{blue}{\frac{\mu}{2}|| w-w^t ||^2}$   
    }
\ENDIF

\IF {method = \textcolor{red}{\emph{FedNova}} }{
    \STATE $\textcolor{red}{\tau_{k}\leftarrow 0}$ 
    }
\ENDIF

\FOR{epoch$=1, 2, \ldots, E$}
    \FOR{batch $b\in \mathcal{B}$}
    
        
        % \STATE $idx$ $\leftarrow$ $Gate(w_g, D)$         \# Pruning stage
        % \STATE $\hat{w} \leftarrow w[idx,:,:...]$       \# select important channels 
        \STATE $w_k^t \leftarrow w_k^t - \eta \triangledown\mathcal{L}(w_k^t,w_g;b)$  \# update neural network
        \STATE $w_g \leftarrow w_g - \eta \triangledown\mathcal{L}(w_k^t,w_g;b)$  \# update pruning gate 
        \IF {method = \textcolor{red}{\emph{FedNova}} }{
            \STATE \textcolor{red}{$\tau_k \leftarrow \tau_k + 1$}
        }
        \ENDIF
    \ENDFOR
 
\ENDFOR
% $idx$ $\leftarrow$ $Gate(w_g, D)$ 

\STATE $\hat{w}^t_k \leftarrow w^t - w_k^t$

\IF{method = \emph{FedAvg} || \textcolor{blue}{\emph{FedProx}} }{
    \STATE return $w_k^t$ to server
}
\ENDIF

\IF {method = \textcolor{red}{\emph{FedNova}} }{
    \STATE return $w_k^t, \textcolor{red}{\tau_{k}}$ to server
    }
\ENDIF
% \STATE return $w, \textcolor{red}{\tau^{c}}$ to server

\end{algorithmic}
\end{algorithm}



==> Content/experiment_figures/f_fednova_dp.tex <==
\begin{figure}[t]
\vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=\columnwidth]{Figures/resnet_fednova.pdf}}
\caption{FedNova with and without Dynamic Pruning.}

\label{fig:dp_fednova}
\end{center}
\vskip -0.2in
\end{figure}

==> Content/experiment_figures/f_resnet.tex <==
\begin{figure}%
    \vskip 0.2in
    \centering
    \subfloat[\centering ResNet-32 without dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/resnet_new.pdf} }}%
    \qquad
    \subfloat[\centering ResNet-32 with dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/resnet_DP_new.pdf} }}%
    \caption{Compare 4 algorithms on ResNet-32.}%
    \label{fig:resnet}%
    \vskip -0.2in
\end{figure}






% \begin{figure}%
% \vskip 0.2in
% \begin{center}
%     \centerline
%     {{\includegraphics[width=\linewidth]{Figures/resnet_new.pdf} }}%
%     \caption{ResNet-32 without Dynamic Pruning.}%
%     \label{fig:resnet}%
% \end{center}
% \vskip -0.2in
% \end{figure}%

==> Content/experiment_figures/f_resnet_dp.tex <==
\begin{figure}%
\vskip 0.2in
\begin{center}
    \centerline
    {{\includegraphics[width=\linewidth]{Figures/resnet_DP_new.pdf} }}%
    \caption{ResNet-32 with Dynamic Pruning.}%
    \label{fig:resnet_dp}%
\end{center}
\vskip -0.2in
\end{figure}%

==> Content/experiment_figures/f_resnet_fed.tex <==
\begin{figure}%
    \centering
    \subfloat[\centering FedAvg.]{{\includegraphics[width=.4\linewidth]{Figures/resnet_fedavg.pdf} }}%
    \qquad
    \subfloat[\centering FedNova.]{{\includegraphics[width=.4\linewidth]{Figures/resnet_fednova.pdf} }}%
    % \caption{ResNet-32 with and without dynamic pruning.}%
    % \label{fig:resnet}%

    \centering
    \subfloat[\centering FedProx.]{{\includegraphics[width=.4\linewidth]{Figures/resnet_fedprox.pdf} }}%
    \qquad
    \subfloat[\centering SCAFFOLD.]{{\includegraphics[width=.4\linewidth]{Figures/resnet_scaffold.pdf} }}%
    
    \caption{Effect of dynamic pruning with 4 algorithm with ResNet-32.}%
    \label{fig:resnet_fed}%
    
    
\end{figure}

==> Content/experiment_figures/f_summary.tex <==
% \begin{figure}%
%     \centering
%     \subfloat[\centering VGG-11 without dynamic pruning.]{{\includegraphics[width=.4\linewidth]{Figures/vgg.pdf} }}%
%     \qquad
%     \subfloat[\centering VGG-11 with dynamic pruning.]{{\includegraphics[width=.4\linewidth]{Figures/vgg_DP.pdf} }}%
%     \caption{Compare 4 algorithms on VGG-11.}%
%     \label{fig:vgg}%
% \end{figure}


% \begin{figure}%
%     \centering
%     \subfloat[\centering ResNet-32 without dynamic pruning.]{{\includegraphics[width=.4\linewidth]{Figures/resnet.pdf} }}%
%     \qquad
%     \subfloat[\centering ResNet-32 with dynamic pruning.]{{\includegraphics[width=.4\linewidth]{Figures/resnet_DP.pdf} }}%
%     \caption{Compare 4 algorithms on ResNet-32.}%
%     \label{fig:resnet}%
% \end{figure}

\begin{figure}%
    \centering
    \subfloat[\centering VGG-11 without dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/vgg_new.pdf} }}%
    \qquad
    \subfloat[\centering VGG-11 with dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/vgg_DP_new.pdf} }}%

    \centering
    \subfloat[\centering ResNet-32 without dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/resnet_new.pdf} }}%
    \qquad
    \subfloat[\centering ResNet-32 with dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/resnet_DP_new.pdf} }}%
    \caption{Comparison of four algorithms on ResNet-32 and VGG-11 models.}%
    \label{fig:summary}%
    
    
\end{figure}

==> Content/experiment_figures/f_vgg11.tex <==

% \begin{figure}%
%     \vskip 0.2in
%     \centering
%     \subfloat[\centering VGG-11 without dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/vgg_new.pdf} }}%
%     \qquad
%     \subfloat[\centering VGG-11 with dynamic pruning.]{{\includegraphics[width=\linewidth]{Figures/vgg_DP_new.pdf} }}%
%     \caption{Compare 4 algorithms on VGG-11.}%
%     \label{fig:vgg}%
%     \vskip -0.2in
% \end{figure}

\begin{figure*}
 \begin{center}

\centerline{\includegraphics[width=\linewidth]{Figures/vgg11_10.pdf}}
\centerline{\includegraphics[width=\linewidth]{Figures/vgg11_30.pdf}}
\centerline{\includegraphics[width=\linewidth]{Figures/vgg11_50.pdf}}
\centerline{\includegraphics[width=\linewidth]{Figures/vgg11_100.pdf}}
\caption{Comparison of 4 algorithms on VGG-11 with and without dynamic pruning on 10, 30, 50 and 100 clients.}



 \vskip -0.3in
\label{fig:vgg11}
\end{center}
 \end{figure*}

==> Content/experiment_figures/f_vgg16.tex <==
% \begin{figure}%
%     \centering
%     \subfloat[\centering FedAvg.]{{\includegraphics[width=.4\linewidth]{Figures/vgg_fedavg.pdf} }}%
%     \qquad
%     \subfloat[\centering FedNova.]{{\includegraphics[width=.4\linewidth]{Figures/vgg_fednova.pdf} }}%

%     \centering
%     \subfloat[\centering FedProx.]{{\includegraphics[width=.4\linewidth]{Figures/vgg_fedprox.pdf} }}%
%     \qquad
%     \subfloat[\centering SCAFFOLD.]{{\includegraphics[width=.4\linewidth]{Figures/vgg_scaffold.pdf} }}%
    
%     \caption{Effect of dynamic pruning with 4 algorithm with VGG-11.}%
%     \label{fig:vgg_fed}%
% \end{figure}

\begin{figure*}
 \begin{center}

\centerline{\includegraphics[width=\linewidth]{Figures/vgg16_10.pdf}}
\centerline{\includegraphics[width=\linewidth]{Figures/vgg16_30.pdf}}
\centerline{\includegraphics[width=\linewidth]{Figures/vgg16_50.pdf}}
\centerline{\includegraphics[width=\linewidth]{Figures/vgg16_100.pdf}}
\caption{Comparison of 4 algorithms on VGG-16 with and without dynamic pruning on 10, 30, 50 and 100 clients.}
 \vskip -0.3in
\label{fig:vgg16}
\end{center}
 \end{figure*}

==> Content/experiment_figures/f_vgg_dp.tex <==
% \begin{figure}[t]
% \vskip 0.2in
% \begin{center}

% \centerline{\includegraphics[width=\columnwidth]{Figures/vgg_DP.pdf}}
% \caption{VGG-11 with Dynamic Pruning.}

% \label{fig:vgg_dp}
% \end{center}
% \vskip -0.2in
% \end{figure}

\begin{figure}%
\vskip 0.2in
\begin{center}
    \centerline
    {{\includegraphics[width=\linewidth]{Figures/vgg_DP_new.pdf} }}%
    \caption{VGG-11 with Dynamic Pruning.}%
    \label{fig:vgg_dp}%
\end{center}
\vskip -0.2in
\end{figure}%

==> Content/experiment_figures/t05_prune_cifar.tex <==
\begin{table}[t]
\caption{Top-1 accuracy results for pruned ResNets on CIFAR-10 and ShuffleNet on CIFAR-100. $\Delta $Top-1 shows the top-1 accuracy gap between the pruned and the original model.}
\label{tab:res_cifar}
% \vspace{-10pt}
\begin{center}
\begin{small}
% \begin{sc}

\begin{tabular}{lccccccr}
\toprule
Model   & Method & FLOPs $\downarrow$  &Top-1 & $\Delta $Top-1 \\
\midrule
\multirow{5}{*}{Res56}     &Uniform& $50\%$   & $87.5$ & $-5.89$ \\
                           &AMC    & $50\%$  & $90.20$ & $-3.19$ \\
                           &FPGM   & $59\%$  & $93.26$ & $-0.02$ \\                           
                           &AGMC   & $50\%$  & $92.00$ & $-1.39$\\
                           &EagleEye   & $50\%$  & $94.66$ & N/A\\
                           &{GNN-RL} & $54\%$ & ${93.49}$ & $ {+0.10}$ \\
% \midrule
% \multirow{3}{*}{ResNet44}    &\multirow{3}{*}{CIFAR-10} &agmc   & $50\%$  &93.10 &  $92.28$ & $-0.82 $ \\
%                              & &rs     & $50\%$  & 93.10&  $ 88.14$ & $-4.96 $ \\
%                              & & {gnn-rl} & $51\%$  &93.10 &  $ {93.23}$ & $ {+0.13}$ \\
\midrule
\multirow{3}{*}{Res32}     &AGMC   & $50\%$ &  $90.96$ & $-1.67$ \\
                           &RS     & $50\%$ &  $ 89.57$ & $-3.06$ \\
                           &SFP     & $42\%$ &  $ 92.08$ & $-0.55$ \\
                           &FPGM     & $50\%$ &  $ 91.93$ & $-0.70$ \\
                           &{GNN-RL} & ${51}$\% & ${92.58}$ & ${-0.05}$ \\
\midrule
\multirow{5}{*}{Res20}    
                          &Uniform& $50\%$ &  $84.00$ & $-7.73$ \\
                          &AMC    & $50\%$ &  $86.40$ & $-5.33$ \\
                          &AGMC   & $50\%$ &  $88.42$ & $-3.31$ \\
                          &SFP   & $42\%$ &  $90.83$ & $-1.37$ \\
                          &FPGM   & $42\%$ &  $91.09$ & $-1.11$ \\
                          &DSA   & $50\%$ &  $91.38$ & $-0.79$ \\
                          & {GNN-RL} & $ {51\%}$   &  ${91.31}$ &  {-0.42} \\


\bottomrule
\end{tabular}
% \end{sc}

\end{small}

\end{center}
\vspace{-15pt}
\end{table}


==> Content/f01_traditional_pruning.tex <==

\begin{figure*}[t]
\vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=0.9\linewidth]{Figures/Traditional_pruning.png}}
\caption{An example of traditional pruning policy under non-IID datasets. The neurons in the neural network reacting differently for two datasets lead to different structures of pruned neural networks.}

\label{fig:tradition_pruning}
\end{center}
\vskip -0.2in
\end{figure*}

==> Content/f03_fl_dp_overview.tex <==


\begin{figure}
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
  \includegraphics[width=\linewidth]{Figures/FedDP.png}

\end{center}
   \caption{Overview of  Federated Learning Pruning (FLP). The dynamic pruning component and the neural network are trained simultaneously when local updating.}


\label{fig:fldp_overview}
\end{figure}

==> Content/f04_Uniform_train.tex <==


\begin{figure}[t]
\vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=\columnwidth]{Figures/details_uniform.pdf}}
\caption{Training details on Uniform pruning policy.}

\label{fig:train_uniform}
\end{center}
\vskip -0.2in
\end{figure}

==> Content/f05_FLP_train.tex <==


\begin{figure}[t]
\vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=\columnwidth]{Figures/details_FLP.pdf}}
\caption{Training details of FLP.}

\label{fig:train_FLP}
\end{center}
\vskip -0.2in
\end{figure}

==> Content/f06_val_acc.tex <==


\begin{figure}[t]
\vskip 0.2in
\begin{center}

\centerline{\includegraphics[width=\columnwidth]{Figures/Accuracy_local_val.pdf}}
\caption{Validation accuracy on pruned VGG-11 under $2\times$ inference acceleration~($50\%$ FLOPs reduction).}

\label{fig:val_acc}
\end{center}
\vskip -0.2in
\end{figure}

==> Content/previous_experiment.tex <==
\subsection{The effect of dynamic pruning on SOTA}


In above section, we equipped the dynamic pruning with SCAFFOLD. In this section, we equip the dynamic pruning with the SOTA and investigate its effectiveness.


In this subsection, we compare the FLP with traditional pruning. Figure~\ref{fig:tradition_pruning} shows the basic idea of the traditional network pruning. The traditional network pruning has the following steps:
\begin{enumerate}
\item Train the original model~(neural network) through federated learning.
\item Perform pruning on the server site. The pruner evaluates the salience of neurons on the neural network and permanently drops those unimportant neurons~(the white neurons in Figure~\ref{fig:tradition_pruning} have been deleted).
\item Pruned neural network send back to local devices.
\item Perform re-training or fine-tuning through federated learning on pruned neural networks to compensate for pruning accuracy loss. 
\end{enumerate}
Since we consider the non-IID dataset in each local device, traditional pruning deploys on each local device would lead to a different neural structure and cause the parameter mismatch when the server aggregates the local model. We perform the traditional pruning on the server site after training and send the pruned model to each device in our experiment setting.
We choose the uniform traditional pruning baselines~\cite{he2017channel}, which prunes the hidden layers with a uniform pruning ratio and delete the convolution channels~(filter) with a low $l^1$-norm value.

Compare to the traditional network pruning, as shown below, the FLP steps are much straightforward:
\begin{enumerate}
\item Deploy dynamic pruning components on each device.
\item Train the neural network and dynamic pruning components together through FL. 
\end{enumerate}
There are two main benefits of FLP. First, we do not need to pre-train the neural network before pruning, and our pruning starts at the run-time. We train the dynamic pruning components together with the neural network. Second, the dynamic pruning components can adaptively select a optimal pruning policy for the non-IID device. 
% However, the universal pruning policy in traditional pruning may sub-optimal for some clients.


% \input{Content/f04_Uniform_train.tex}
% \input{Content/experiment_figures/f_vgg.tex}
% \input{Content/experiment_figures/f_vgg_dp.tex}
% \input{Content/experiment_figures/f_summary.tex}
% \input{Content/experiment_figures/f_resnet.tex}
% \input{Content/experiment_figures/f_resnet_dp.tex}



% Figure~\ref{fig:train_uniform} and~\ref{fig:train_FLP} shows the training details of traditional pruning and FLP. Both the FLP and traditional pruning prune 50\% FLOPs~(floating point operations per second) on the VGG-11~\cite{Simonyan2015VGG}. 

Figure~\ref{fig:vgg} shows the training details on VGG-11 with and without pruning on all four FL algorithms. Figure~\ref{fig:resnet} shows the training details on ResNet-32 with and without pruning on all four FL algorithms. As shown in the these figures, FLP reduces communication round to reach the target accuracy~($78\%$) in all algorithms except \emph{FedAvg}. The result is summarized in Table~\ref{com_rounds}.


% Table~\ref{bandwidth} shows the bandwidth communicated between clients and server.



The total FLOPs consumption of our best performing method (\emph{SCAFFOLD}) with and without dynamic pruning is recorded in Table~\ref{flops}.  The original VGG-11 has 15.48 billion FLOPs and under $2\times$ acceleration, we reduced 7.36 billions FLOPs~($50\%$ FLOPs compared to the original model). Similarly, the FLOPs of ResNet-32 has been reduced from 7.36 billions to 3.68 billions.

The total communication cost when training the VGG-11~\cite{simonyan2015vgg} and ResNet-32~\cite{he2016resnet} is recorded in table~\ref{bandwidth}. We have applied the FLP on various FL methods. The results show our approach can significantly reduce the communication cost on all the FL methods. Especially, on FedProx~\cite{li2020fedprox}, by applying the FLP,  66650 MB communication cost had been reduced, which is $2 \times$ less cost than the original FedProx. Additionally, we found the FLP achieves the best performance on the SCAFFOLD~\cite{karimireddy2020scaffold}, where to train the VGG-11 and ResNet-32 only take 20767 MB and 3662 MB communication cost respectively, which is significantly superior to others.


\input{Content/t03_bandwidth}

% The total communication cost of our best performing method (\emph{SCAFFOLD}) with and without dynamic pruning is recorded in Table~\ref{bandwidth}. The function for computing the cost is defined as: $\text{Cost} = \text{Number of Parameters} \times \text{Rounds to reach target accuracy} \times \text{Number of clients} \times \text{Percentage of clients participating each round}$. As can be seen in Table~\ref{bandwidth}, FLP helps to reduce more than $14\%$ for VGG-11 and $29\%$ for ResNet-32.


% Additionally, the computation cost of the pruning components on each local device is negligible. The total FLOPs consumption of pruning components on VGG-11 is $1.024$ Million FLOPs since the pruning components are essentially linear layers. However, the original VGG-11 has 8 Billion FLOPs. Under $2\times$ acceleration, we reduced 4 Billion FLOPs~($50\%$ FLOPs compared to the original model) and only added $1.024$ million extra FLOPs to decide the pruning policy.

% As shown in Figure~\ref{fig:train_uniform}, the traditional pruning starts pruning when we finish training the original neural network~(starts at the 75 rounds), and the pruning will cause the accuracy loss.
% To get the $78\%$ test accuracy, the model with a traditional pruning will need 19 extra rounds to compensate for the accuracy loss, a total of 94 rounds. This result in Figure~\ref{fig:train_uniform} is based on the Unifrom tradition pruning policy. However, it can be extended to all traditional pruning methods because they require trained neural network information to generate a pruning policy. So even the SOTA pruning methods need extra rounds to compensate for accuracy loss.

% As Figure~\ref{fig:train_FLP} shows, the FLP only need 73 rounds to get the $78\%$ test accuracy and $50\%$ FLOPs reduction, and no extra rounds are needed to compensate for the test accuracy loss.

% Table~\ref{summary} summarizes the communication cost needed to attain a target of $78\%$ average accuracy. FLP reduces communication round to reach the target accuracy in all algorithms except  \emph{FedAvg}. 

% We stress that these already quite sizeable gains are obtained in the non-IID case, and can be expected to grow when the imbalance grows, as testified by the performance gap in the extreme disjoint case.

% \input{Content/f05_FLP_train.tex}
% Compare to the traditional pruning method, Uniform pruning method for instance, The FLP are more 

% \subsection{Inference acceleration and local accuracy}
% \input{Content/t02_inference_acc}
% \input{Content/f06_val_acc}
% This section evaluates the FLP by inference and accuracy and compares it with the traditional uniform pruning policy. Since inference varies among different devices, we use the floating-point operations per second~(FLOPs) to evaluate the inference of neural networks.
% The FLP produces the dataset-aware pruning policy for each local device. To test the pruning policy, for each device, we split non-IID local validation datasets for clients from the test set. Each local validation set has 1000 pictures.


% Figure~\ref{fig:val_acc} shows the validation accuracy of $50\%$ FLOPs VGG-11 pruned by uniform traditional pruning baseline and the FLP. On the total 10 clients, we outperform the traditional uniform pruning policy in most of the case. 
% Additionally, the computation cost of the pruning components on each local device is negligible. The total FLOPs consumption of pruning components on VGG-11 is $1.024$ Million FLOPs since the pruning components are essentially linear layers. However, the original VGG-11 has 8 Billion FLOPs. Under $2\times$ acceleration, we reduced 4 Billion FLOPs~($50\%$ FLOPs compared to the original model) and only added $1.024$ million extra FLOPs to decide the pruning policy.

% \subsubsection{Time measurement}
% The effectiveness of model pruning on edge devices is demonstrated by time measurement of the FL system. We use the full-size VGG-11 model and measure the averaged time elapsed of FL on these pruned models involving both the server and clients.
% Figure~\ref{fig:communication_time} shows that the communication time decreases as number of FLOPs decreases.


% \subsection{Pruning enable efficient FL}

% \subsubsection{Bandwidth \& communication cost}
% We compare all four FL algorithms~(FedAvg, FedProx, Scaffold, FedNova) with and without pruning with CIFAR-10 dataset on VGG-11 and VGG-16. In Figure~\ref{fig:dp_fednova}, we use the FedNova~\cite{wang2020fednova} algorithm to train the ResNet-32. The figure shows the comparison between training the full ResNet-32 model and training the  federated learning rounds and corresponding bandwidth consumption. The dynamic pruning do not hurt the training process of the training.

% the bandwidth of each algorithm after reaching ..\% accuracy. Although FLP needs more rounds to reach target accuracy, the model size in each client is much smaller.

%VGG-11 and VGG-16 on Cifar-10 with FedAvg with and without pruning, FedNova, .... with and without pruning.

% \subsubsection{Inference acceleration}
%bar chart, expect all client have less time w/ pruning compared to w/t pruning.
% In Figure~\ref{fig:dp_fednova}, FLP indicates a clear benefit of faster inference time versus without pruning. Our methods have reduced the time by ...\%.


% \subsection{Comparison with other pruning methods}
% We experiment with FLP and compare its accuracy vs. round curve with (i) conventional FL, (ii) PruneFL and (iii) SNIP. We implement Conv-2 model for FEMNIST, VGG-11 for CIFAR-10 and ResNet18 for ImageNet.


% \subsubsection{Training time and accuracy}
% The training time~(rounds) needed to reach ...\% accuracy are recorded in Figure~\cite{training_time_all} while the converged accuracies are recorded in
% Figure~\cite{converged_accuracy_all}. As we can see from these figures, FLP requires lesser time to reach target ...\% and converges at a higher accuracy.


%First figure about time needed to reach target accuracy
%Second figure about comparing converged accuracy
% \subsubsection{Bandwidth and communication cost}
% Figure~\cite{bandwidth_all} shows the bandwidth reduction of FLP over other pruning methods at 100 rounds.

% Use one figure to compare different pruning methods (each method is one curve) -- like figure 1 in the baseline paper (PruneFL, SNIPS, iterative FL, ....) 


% \subsubsection{Each client accuracy with non-IID}
%bar chart/ table.
% Figure~\cite{client_niid} shows the accuracy improvement on each client with FLP comparing with other pruning methods.

% \subsection{Inference acceleration}
% Since inference varies among different devices, here we use the floating point operations per second~(FLOPs) to evaluate the inference of nueral networks.



% The details of the datasets are summarized in Table \ref{tab:dataset}.



 
% We used VGG-11~\cite{simonyan2015deep} for the model and the classic \emph{FedAvg} for federated setting. In each communication round, the current version of the model will be sent to all 10 clients. Then these clients will run stochastic gradient descent (SGD) to do local update at each client and we will aggregate the update. The global objective (loss) function is a weighted average of local objectives in proportion of their data-size:

% \begin{gather*}
%     F(\textbf{w}) = \sum_{k=1}^{K}p_k F_k(\textbf{w})\\
%     \text{where } p_k = \frac{|S_k|}{\sum_{k=1}^{K}|S_k|}\\
% \end{gather*}

% Where $F_k(\textbf{w})$ is client $k$'s loss function. $|S_k|$ is size of client $k$'s dataset. So clients with larger dataset will have correspondingly larger losses.


% The configuration of experiment are summarized in Table \ref{tab:config}.






% \begin{figure}
%     \centering
%     \includegraphics[width=15cm]{partition.png}
%     \caption{\textbf{The distribution of CIFAR-10 in the experiments.}}
%     \label{fig:partition}
% \end{figure}


% Table generated by Excel2LaTeX from sheet 'Sheet1'
% \begin{table}[htbp]
%   \centering
%   \caption{\textbf{The distribution of CIFAR-10 in the experiments.}}
%     \begin{tabular}{lcccccccccc}
%     % \multicolumn{11}{c}{\textbf{Label}} \\
%     % \midrule
%     \toprule
%         & \emph{Airplane} & \emph{Automobile} & \emph{Bird} & \emph{Cat} & \emph{Deer} & \emph{Dog} & \emph{Frog} & \emph{Horse} & \emph{Ship} & \emph{Truck} \\
%     \midrule
%     \emph{Client 0} & 0   & 75  & 2995 & 695 & 8   & 5   & 0   & 309 & 9   & 0 \\
%     \midrule
%     \emph{Client 1} & 790 & 4   & 1327 & 979 & 2574 & 0   & 0   & 0   & 0   & 0 \\
%     \midrule
%     \emph{Client 2} & 2608 & 587 & 534 & 14  & 194 & 0   & 6   & 493 & 98  & 0 \\
%     \midrule
%     \emph{Client 3} & 0   & 0   & 74  & 3   & 3   & 37  & 0   & 0   & 288 & 71 \\
%     \midrule
%     \emph{Client 4} & 5   & 0   & 9   & 2   & 0   & 10  & 556 & 11  & 0   & 4459 \\
%     \midrule
%     \emph{Client 5} & 0   & 0   & 1   & 0   & 0   & 0   & 0   & 4183 & 1072 & 0 \\
%     \midrule
%     \emph{Client 6} & 0   & 4220 & 0   & 0   & 2   & 113 & 0   & 0   & 3532 & 0 \\
%     \midrule
%     \emph{Client 7} & 0   & 5   & 59  & 443 & 867 & 4665 & 0   & 0   & 0   & 0 \\
%     \midrule
%     \emph{Client 8} & 771 & 83  & 0   & 2863 & 983 & 154 & 857 & 0   & 0   & 0 \\
%     \midrule
%     \emph{Client 9} & 826 & 26  & 1   & 1   & 369 & 16  & 3581 & 4   & 1   & 470 \\
%     \bottomrule
%     \end{tabular}%
%   \label{tab:partition}%
% \end{table}%




% \subsection{Bandwidth}

% The model size are recorded in Table \ref{tab:modelsize}.


% \begin{table}[h!]
%     \begin{center}
%     \caption{\textbf{The model size in the experiments.}}
%     \label{tab:modelsize}
%     \begin{tabular}{ccc}
%     \toprule
%     \emph{Original VGG-11} & \emph{75\% FLOPs VGG-11} & \emph{50\% FLOPs VGG-11} \\
%     \midrule
%     38 Mb & 30 Mb & 22 Mb \\
%     \bottomrule
%     \end{tabular}
%     \end{center}
% \end{table}









% \subsection{Global accuracy}

% Testing accuracy of the all three models on CIFAR-10 dataset is shown in Figure \ref{fig:cifar10_test_all}. 


% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=10cm]{cifar10_test_all.jpg}
%     \caption{\textbf{Testing accuracy of all three models on CIFAR-10.}}
%     \label{fig:cifar10_test_all}
% \end{figure}


% \begin{figure}[htp]
%     \centering
%     % \includegraphics[width=10cm]{original-cifar10-test.jpg}
%     \caption{\textbf{Testing accuracy of model on CIFAR-10.}}
%     \label{fig:original-cifar10-test}
% \end{figure}

% \subsection{Inference time}

% The performance of model with static pruning 50\% channels is shown in Figure \ref{fig:static50-cifar10-test}. 

% \begin{figure}[htp]
%     \centering
%     \includegraphics[width=10cm]{static50-cifar10-test.jpg}
%     \caption{\textbf{Testing accuracy of 50\% model on CIFAR-10.}}
%     \label{fig:static50-cifar10-test}
% \end{figure}


==> Content/table/t01_com_rounds.tex <==

% \begin{table}
%   \caption{Communication round to reach 78\% accuracy}
%   \label{table}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
% \end{table}


\begin{table}
  \caption{Communication rounds to reach 78\% accuracy.}
  \label{com_rounds}
  \centering
  \begin{tabular}{cccc}
    \toprule
    Model & Algorithm & Original & FLP \\
    \midrule
    VGG-11 & FedAvg   & 74   & >100   \\
    VGG-11 & FedProx  & >100 & 71     \\
    VGG-11 & FedNova  & 62   & 38     \\
    VGG-11 & SCAFFOLD & 28   & 24     \\
    ResNet-32 & FedAvg   & 76   & >100  \\
    ResNet-32 & FedProx  & >100 & 74    \\
    ResNet-32 & FedNova  & 62   & 58    \\
    ResNet-32 & SCAFFOLD & 34   & 24   \\
    \bottomrule
  \end{tabular}
\end{table}

==> Content/table/t01_training_details.tex <==
\begin{table}
    \begin{center}
    \caption{Training settings.}
    \label{tab:config}
    \begin{tabular}{ccccc}
    \toprule
    \emph{Optimizer} & \emph{Learning rate} & \emph{Batch size} & \emph{Epoch} & \emph{Number of clients}\\
    \midrule
    SGD & 0.1 & 64 & 10 & 10\\
    \bottomrule
    \end{tabular}
  \end{center}
\end{table}

==> Content/table/t02_inference_acc.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table}[htbp]
  \centering
  \caption{Pruned VGG-11 val. accuracy on local Non-IID dataset}
    \begin{tabular}{lccc}
    \toprule
        & \emph{FLOPs} & \emph{Uniform} Acc. & \emph{FLP} Acc.\\
    \midrule
    \emph{Client 0}  &$51\% (2\times)$& 80.05\% & 82.11\% \\
    \midrule
    \emph{Client 1}    &$51\% (2\times)$& 73.69\% & 86.70\% \\
    \midrule
    \emph{Client} 2    &$51\% (2\times)$& 73.28\% & 86.49\% \\
    \midrule
    \emph{Client 3}    &$51\% (2\times)$& 82.66\% & 88.31\% \\
    \midrule
    \emph{Client 4}  &$51\% (2\times) $& 72.03\% & 84.29\% \\
    \midrule
    \emph{Client 5}   &$51\% (2\times)$& 74.13\% & 72.97\% \\
    \midrule
    \emph{Client 6}   &$51\% (2\times)$& 77.54\% & 82.70\% \\
    \midrule
    \emph{Client 7}  &$51\% (2\times) $ & 76.80\% & 87.41\% \\
    \midrule
    \emph{Client 8}  &$51\% (2\times)$  & 71.97\% &82.04\% \\
    \midrule
    \emph{Client 9}   &$51\% (2\times)$ & 72.12\% & 80.72\% \\
    \bottomrule
    \end{tabular}%
  \label{tab:accuracy}%
\end{table}%

==> Content/table/t03_bandwidth.tex <==
\begin{table}
  \caption{Communication cost for various model to reach 78\% accuracy (MB).}
  \label{tab:bandwidth}
  \centering
  \begin{tabular}{ccccc}
    \toprule
    Model &FL method & Model size & {Comm. cost}\\
    \midrule
    
    VGG-11  & FedProx& 132.86 &  $132860$ \\
    VGG-11  & FedProx + FLP& 93.00 &  $66030$ \\
    
    VGG-11  & FedNova& 132.86 &  $82373$ \\
    VGG-11  & FedNova + FLP& 93.00 &  $35340$ \\
    
    VGG-11  & SCAFFOLD& 132.86 &  $37200$ \\
    VGG-11  & \textbf{SCAFFOLD + FLP} & 93.00 &  \textbf{20767} \\
    
  
    
    ResNet-32  & FedProx & 21.80 &  $21800$ \\
    ResNet-32  & FedProx + FLP & 15.26 &  $11292$ \\
    
    ResNet-32  & FedNova & 21.80 &  $13516$ \\
    ResNet-32  & FedNova + FLP & 15.26 &  $8850$  \\
    
    ResNet-32  & SCAFFOLD & 21.80 &  $7412$ \\
    ResNet-32  & \textbf{SCAFFOLD + FLP} & 15.26 &  \textbf{3662}   \\
    \bottomrule
  \end{tabular}
\end{table}

==> Content/table/t04_train_effi.tex <==

\begin{table}
  \caption{Communication rounds to reach 78\% accuracy.}
  \label{tab:train_eff}
  \centering
  \begin{tabular}{cccc}
    \toprule
    Model & Algorithm & Rounds & Comm. cost \\
    \midrule
    \multirow{4}{*}{VGG-11} & FedAvg   & 74   & >100   \\
     & FedProx  & >100 & 71     \\
     & FedNova  & 62   & 38     \\
     & SCAFFOLD & 28   & 24     \\
    \multirow{4}{*}{ResNet-32} & FedAvg   & 76   & >100  \\
     & FedProx  & >100 & 74    \\
     & FedNova  & 62   & 58    \\
     & SCAFFOLD & 34   & 24   \\
        \multirow{4}{*}{ResNet-20} & FedAvg   & -   & -  \\
     & FedProx  & - & -    \\
     & FedNova  & -   & -    \\
     & SCAFFOLD & -   & -   \\
    \bottomrule
  \end{tabular}
\end{table}

==> Content/table/t_converge.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Comparison of communication cost with SoTAs to achieve model convergence.}
\label{tab:com_cost2}
\resizebox{\textwidth}{!}{%
\begin{tabular}{cccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Clients}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Sample \\ Ratio\end{tabular}}} & \multirow{2}{*}{\textbf{Converge Rounds}} & \multicolumn{3}{c}{\textbf{Communication Cost}}             & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Avg.\\ Converge Acc.\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}$\Delta$ \\ Acc.\end{tabular}}} \\
                                 &                                 &                                   &                                                                                   &                                           & \textbf{Round/Client}   & \textbf{Total} & \textbf{Speedup} &                                                                                        &                                                                                    \\ \hline
\multirow{5}{*}{FedAvg~\cite{mcmahan2017fedavg}}          & \multirow{2}{*}{ResNet-20}      & 30                                & 0.4                                                                               & 170                                       & \multirow{2}{*}{2.1MB}  & 4.18GB         & (1 $\times$)     & 60.58\%                                                                                & 0\%                                                                                \\
                                 &                                 & 50                                & 0.7                                                                               & 184                                       &                         & 13.21GB        & (1 $\times$)     & 32.71\%                                                                                & 0\%                                                                                \\
                                 & ResNet-32                       & 30                                & 0.4                                                                               & 140                                       & 3.2MB                   & 5.25GB         & (1 $\times$)     & 64.92\%                                                                                & 0\%                                                                                \\
                                 & \multirow{2}{*}{VGG-11}         & 50                                & 0.7                                                                               & 171                                       & \multirow{2}{*}{42MB}   & 246GB          & (1 $\times$)     & 32.68\%                                                                                & 0\%                                                                                \\
                                 &                                 & 100                               & 0.4                                                                               & 322                                          &                         &          528GB      & (1 $\times$)     &      28.33\%                                                                                  & 0\%                                                                                \\ \hline
\multirow{5}{*}{FedNova~\cite{wang2020fednova}}         & \multirow{2}{*}{ResNet-20}      & 30                                & 0.4                                                                               & 159                                       & \multirow{2}{*}{4.2MB}  & 7.83GB         & (0.54 $\times$)  & 64.50\%                                                                                & +3.92\%                                                                            \\
                                 &                                 & 50                                & 0.7                                                                               & 200                                       &                         & 28.71GB        & (0.46 $\times$)  & 38.35\%                                                                                & +5.64\%                                                                            \\
                                 & ResNet-32                       & 30                                & 0.4                                                                               & 149                                       & 6.4MB                   & 11.18GB        & (0.47 $\times$)  & 67.48\%                                                                                & +2.56\%                                                                            \\
                                 & \multirow{2}{*}{VGG-11}         & 50                                & 0.7                                                                               & 193                                       & \multirow{2}{*}{84MB}   & 554GB          & (0.44 $\times$)  & 29.90\%                                                                                & -2.78\%                                                                            \\
                                 &                                 & 100                               & 0.4                                                                               & 287                                          &                         &       941GB         & (0.56 $\times$)     &     22.12\%                                                                                   &     -6.21\%                                                                               \\ \hline
\multirow{5}{*}{FedProx~\cite{li2020fedprox}}         & \multirow{2}{*}{ResNet-20}      & 30                                & 0.4                                                                               & 157                                       & \multirow{2}{*}{2.1MB}  & 3.86GB         & (1.08 $\times$)  & 60.20\%                                                                                & -0.38\%                                                                            \\
                                 &                                 & 50                                & 0.7                                                                               & 193                                       &                         & 13.85GB        & (0.95 $\times$)  & 32.43\%                                                                                & -0.28\%                                                                            \\
                                 & ResNet-32                       & 30                                & 0.4                                                                               & 151                                       & 3.2MB                   & 5.66GB         & (0.93 $\times$)  & 64.75\%                                                                                & -0.17\%                                                                            \\
                                 & \multirow{2}{*}{VGG-11}         & 50                                & 0.7                                                                               & 195                                       & \multirow{2}{*}{42MB}   & 280GB          & (0.88 $\times$)  & 32.14\%                                                                                & -0.54\%                                                                            \\
                                 &                                 & 100                               & 0.4                                                                               & 123                                          &                         &        201GB        & (2.63 $\times$)     &      31.21\%                                                                                  &      +2.88\%                                                                              \\ \hline
\multirow{5}{*}{SCAFFOLD~\cite{karimireddy2020scaffold}}        & \multirow{2}{*}{ResNet-20}      & 30                                & 0.4                                                                               & 400                                       & \multirow{2}{*}{4.3MB}  & 20.16GB        & (0.20 $\times$)  & 10.00\%                                                                                   & -50.58\%                                                                           \\
                                 &                                 & 50                                & 0.7                                                                               & 400                                       &                         & 58.79GB        & (0.22 $\times$)  & 10.00\%                                                                                   & -22.71\%                                                                           \\
                                 & ResNet-32                       & 30                                & 0.4                                                                               & 400                                       & 6.5MB                   & 30.47GB        & (0.17 $\times$)  & 10.00\%                                                                                   & -54.92\%                                                                           \\
                                 & \multirow{2}{*}{VGG-11}         & 50                                & 0.7                                                                               & 400                                       & \multirow{2}{*}{84MB}   & 1148GB         & (0.21 $\times$)  & 10.00\%                                                                                   & -22.68\%                                                                           \\
                                 &                                 & 100                               & 0.4                                                                               & 400                                       &                         &      1312GB          & (0.40 $\times$)     & 31.78\%                                                                                   &      +3.45\%                                                                              \\ \hline
\multirow{5}{*}{SPATL (Ours)}    & \multirow{2}{*}{ResNet-20}      & 30                                & 0.4                                                                               & 140                                       & \multirow{2}{*}{2.1MB}  & 3.44GB         & (1.21 $\times$)  & 66.49\%                                                                                & +5.91\%                                                                            \\
                                 &                                 & 50                                & 0.7                                                                               & 171                                       &                         & 12.27GB        & (1.08 $\times$)  & 42.54\%                                                                                & +9.83\%                                                                            \\
                                 & ResNet-32                       & 30                                & 0.4                                                                               & 117                                       & 3.6MB                   & 4.93GB         & (1.06 $\times$)  & 70.23\%                                                                                & +5.31\%                                                                            \\
                                 & \multirow{2}{*}{VGG-11}         & 50                                & 0.7                                                                               & 156                                       & \multirow{2}{*}{61.3MB} & 324GB          & (0.76 $\times$)  & 49.76\%                                                                                & +17.08\%                                                                           \\
                                 &                                 & 100                               & 0.4                                                                               & 86                                          &                         &        205GB        & (2.58 $\times$)     &      44.23\%                                                                                  &     +15.90\%                                                                               \\ \hline
\end{tabular}%
}
\end{table*}

==> Content/table/t_training_cost.tex <==
% Please add the following required packages to your document preamble:
%  \usepackage{multirow}
%  \usepackage{graphicx}
\begin{table*}[]
\centering
\caption{Comparison of communication cost with SoTAs to achieve 80\% accuracy.}
\label{tab:com_cost}
\resizebox{\textwidth}{!}{%
\begin{tabular}{ccccccccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Target\\ Accuracy\end{tabular}}} & \multirow{2}{*}{\textbf{Clients}} & \multirow{2}{*}{\textbf{Communication Rounds}} & \multicolumn{4}{c}{\textbf{Communication Cost}}                                     \\
                                 &                                 &                                                                                     &                                   &                                                & \textbf{Round/Client} & \textbf{Total} & \textbf{$\Delta$ Cost} & \textbf{Speed Up} \\ \hline
\multirow{3}{*}{FedAvg~\cite{mcmahan2017fedavg}}          & ResNet-20                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 203                                            & 2.1MB                 & 4.16GB         & 0GB                    & (1 $\times$)      \\
                                 & ResNet-32                       &                                                                                     &                                   & 192                                            & 3.2MB                 & 6.00GB         & 0GB                    & (1 $\times$)      \\
                                 & VGG-11                          &                                                                                     &                                   & 181                                            & 42MB                  & 74.24GB        & 0GB                    & (1 $\times$)      \\ \hline
\multirow{3}{*}{FedNova~\cite{wang2020fednova}}         & ResNet-20                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 198                                            & 4.2MB                 & 8.12GB         & +3.96GB                & (0.51 $\times$)   \\
                                 & ResNet-32                       &                                                                                     &                                   & 197                                            & 6.4MB                 & 12.31GB        & +6.31GB                & (0.48 $\times$)   \\
                                 & VGG-11                          &                                                                                     &                                   & 159                                            & 84MB                  & 130.43GB       & +56.19                 & (0.57 $\times$)   \\ \hline
\multirow{3}{*}{FedProx~\cite{li2020fedprox}}         & ResNet-20                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 288                                            & 2.1MB                 & 5.91GB         & +1.75GB                & (0.70 $\times$)   \\
                                 & ResNet-32                       &                                                                                     &                                   & 400                                            & 3.2MB                 & 12.80GB        & +6.80GB                & (0.47 $\times$)   \\
                                 & VGG-11                          &                                                                                     &                                   & 296                                            & 42MB                  & 121.41GB       & +47.17GB               & (0.61 $\times$)   \\ \hline
\multirow{3}{*}{SCAFFOLD~\cite{karimireddy2020scaffold}}        & ResNet-20                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 49                                             & 4.3MB                 & 2.10GB         & -2.06GB                & (1.98 $\times$)   \\
                                 & ResNet-32                       &                                                                                     &                                   & 55                                             & 6.5MB                 & 3.60GB         & -2.40GB                & (1.67 $\times$)   \\
                                 & VGG-11                          &                                                                                     &                                   & 54                                             & 84MB                  & 45.00GB        & -29.24GB               & (1.65 $\times$)   \\ \hline
\multirow{3}{*}{FedDP (Ours)}    & ResNet-20                       & \multirow{3}{*}{80\%}                                                               & \multirow{3}{*}{10}               & 52                                             & 2.1MB                 & 1.10GB         & -3.06GB                & (3.78 $\times$)   \\
                                 & ResNet-32                       &                                                                                     &                                   & 50                                             & 3.6MB                 & 1.80GB         & -4.20GB                & (3.33 $\times$)   \\
                                 & VGG-11                          &                                                                                     &                                   & 36                                             & 84MB                & 30.24GB        & -44.00GB               & (2.46 $\times$)   \\ \hline
\end{tabular}%
}
\end{table*}
